Towards Diverse Device Heterogeneous Federated Learning via Task Arithmetic Knowledge Integration

Federated Learning has emerged as a promising paradigm for collaborative machine learning, while preserving user data privacy. Despite its potential, standard FL lacks support for diverse heterogeneous device prototypes, which vary significantly in model and dataset sizes -- from small IoT devices to large workstations. This limitation is only partially addressed by existing knowledge distillation techniques, which often fail to transfer knowledge effectively across a broad spectrum of device prototypes with varied capabilities. This failure primarily stems from two issues: the dilution of informative logits from more capable devices by those from less capable ones, and the use of a single integrated logits as the distillation target across all devices, which neglects their individual learning capacities and and the unique contributions of each. To address these challenges, we introduce TAKFL, a novel KD-based framework that treats the knowledge transfer from each device prototype's ensemble as a separate task, independently distilling each to preserve its unique contributions and avoid dilution. TAKFL also incorporates a KD-based self-regularization technique to mitigate the issues related to the noisy and unsupervised ensemble distillation process. To integrate the separately distilled knowledge, we introduce an adaptive task arithmetic knowledge integration process, allowing each student model to customize the knowledge integration for optimal performance. Additionally, we present theoretical results demonstrating the effectiveness of task arithmetic in transferring knowledge across heterogeneous devices with varying capacities. Comprehensive evaluations of our method across both CV and NLP tasks demonstrate that TAKFL achieves SOTA results in a variety of datasets and settings, significantly outperforming existing KD-based methods Code is released at https://github.com/MMorafah/TAKFL

==> algorithms.tex <==
\section{Algorithms}


\begin{algorithm}[H]
\caption{Federated Learning}
\label{alg:FedAvg}

% \DontPrintSemicolon
% \SetCommentSty{mycommfont}
% \SetAlgoLined
% \SetKwInOut{Req}{Require}
% \SetKwFunction{FClient}{ClientUpdate}
% \SetKwProg{Fn}{}{:}{}

\begin{algorithmic}[1]
\REQUIRE number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$).
%\SetKwProg{Fn}{Server Executes}{:}{}
\STATE \textbf{Server Executes:}
\STATE Initialize the server model with $\btheta_g^0$ \;
\FOR {each round $t = 0, 1, \ldots, T-1$}
\STATE $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
\STATE $S_t \leftarrow $(random set of m clients) \; %\tcp*{set of $m$ available clients}
\FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
\STATE $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
%$\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
\ENDFOR
\STATE $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
\ENDFOR
\vspace{1mm}
\FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
\STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
\STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k^{train}$ into batches of Size $B$})\;
\FOR {each local epoch $ \in \{1, \ldots, E\}$}
\FOR {each batch $\mathbf{b} \in \mathcal{B}$}
\STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} \ell(f_k(\bx; \btheta^{t}_k), y)$\;
\ENDFOR
\ENDFOR
\STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
\ENDFUNCTION
% \Fn{\FClient{$k, \btheta^t_{g}$}}{
%     \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
%     \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
%     \For {each local epoch $i = 1, \dots, E$} {
%         \For {each batch $\mathbf{b} \in \mathcal{B}$} {
%             \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} f_k(\btheta^{t}_k; \mathbf{b})$\;
%         }
%     }
%     \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
%     \KwRet $\btheta^{t+1}_{k}$\;
% }
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[H]
% \caption{FedAvg}
% \label{alg:FedAvg}

% % \DontPrintSemicolon
% % \SetCommentSty{mycommfont}
% % \SetAlgoLined
% % \SetKwInOut{Req}{Require}
% % \SetKwFunction{FClient}{ClientUpdate}
% % \SetKwProg{Fn}{}{:}{}

% \begin{algorithmic}[1]
% \STATE \textbf{Require:} number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$).
% %\SetKwProg{Fn}{Server Executes}{:}{}
% \STATE \textbf{Server Executes:}
% \STATE $\quad$ Initialize the server model with $\btheta_g^0$ \;
% \FOR {each round $t = 0, 1, \dots, T-1$}
% \STATE $\quad$ $m \leftarrow {\rm{max}}(C \cdot N,1)$ \;
% \STATE $\quad$ $S_t \leftarrow $(random set of m clients) \; %\tcp*{set of $m$ available clients}
% $\quad$ \FOR {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% \STATE $\quad$ $\btheta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \btheta^t_{g} )$ \; 
% %$\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% \ENDFOR
% \STATE $\quad$ $\btheta^{t+1}_{g}=\mathtt{ModelFusion}(\{\btheta_k \}_{k \in S_t})$
% \ENDFOR
% \vspace{1mm}
% \FUNCTION {$\mathtt{ClientUpdate}(k, \btheta^t_{g})$}
% \STATE H
% \ENDFUNCTION
% % \Fn{\FClient{$k, \btheta^t_{g}$}}{
% %     \STATE $\btheta^{t}_k \leftarrow \btheta^t_{g}$ \;
% %     \STATE $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
% %     \For {each local epoch $i = 1, \dots, E$} {
% %         \For {each batch $\mathbf{b} \in \mathcal{B}$} {
% %             \STATE $\btheta^{t}_k \leftarrow \btheta^{t}_k - \eta \nabla_{\btheta^{t}_k} f_k(\btheta^{t}_k; \mathbf{b})$\;
% %         }
% %     }
% %     \STATE $\btheta^{t+1}_k \leftarrow \btheta^{t}_k$\;
% %     \KwRet $\btheta^{t+1}_{k}$\;
% % }
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{FedProx}
% \label{alg:FedProx}

% \DontPrintSemicolon
% \SetCommentSty{mycommfont}
% \SetAlgoLined
% \SetKwInOut{Req}{Require}
% \SetKwFunction{FClient}{ClientUpdate}

% \Req{number of clients ($N$), sampling rate ($C\in(0,1]$), number of communication rounds ($T$), 
% local dataset of client $k$ ($D_k$), number of local epoch ($E$), number of local batch size ($B$), learning rate ($\eta$), FedProx parameter ($\mu$)\;}
% \SetKwProg{Fn}{Server Executes}{:}{}
% \Fn{}{
% Initialize the server model with $\theta_g^0$ \;
% \For {each round $t = 0, 1, \dots, T-1$} {
%  $m \leftarrow {\rm{max}}(C \cdot N,1)$\;
%  $S_t \leftarrow $(random set of m clients)\; %\tcp*{set of $m$ available clients}
% \For  {each client $k \in S_t$ \rm{\textbf{in parallel}}}
% { 
% $\theta^{t+1}_{k}\leftarrow {\mathtt{ClientUpdate}}(k; \theta^t_{g} )$ \; 
% }

% $\theta^{t+1}_{g}=\sum_{k \in S_t }{|D_{k}|\theta^{t+1}_{k}}  /\sum_{k \in S_t }{|D_{k}|}$
% }
% }
% %\Indm
% \SetKwProg{Fn}{}{:}{}
% \Fn{\FClient{$k, \theta^t_{g}$}}{
%      $\theta^{t}_k \leftarrow \theta^t_{g}$\;
%      $\mathcal{B} \leftarrow$ ({randomly splitting $D_k$ into batches of Size $B$})\;
%     \For {each local epoch $i = 1, \dots, E$} {
%         \For {each batch $\mathbf{b} \in \mathcal{B}$} 
%         {
%              $\theta^{t+1}_k \leftarrow \argmin_{\theta_k} \mathbb{E} \left[ f(\theta_k; \mathbf{b}) \right] + \frac{\mu}{2} ||\theta_k - \theta^t_k||^2$\;
%         }
%     }
%     $\theta^{t+1}_k \leftarrow \theta^{t}_k$\;
%     \KwRet $\theta^{t+1}_{k}$\;
% }
% \end{algorithm}



==> nsecs/background1.tex <==
\section{Background and Problem Definition}\label{sec:problem} %(Device Diversity Federated Learning Problem)
%In this section, we formally define the FL-H5 problem.
\subsection{Background and Notations}
\textbf{Vanilla FedAvg.} Suppose there is a set of clients $S$, where each client $k$ has local dataset $D_k$. The entire clients participate in federating learning process to train a machine learning model $f(\cdot; \btheta)$ over the whole dataset $\cD = \bigcup_{k=1}^{\l S\l} \cD_k$ under orchestration of a central server while preserving the privacy of local datasets. At each round $r$, $C \in (0, 1]$ fraction of clients are being randomly selected denoted as $S_r$. The $S_r$ selected clients receive the current parameters of global model $\btheta_r^g$ and locally train it. Then, they send back their updated parameters $\{{\widehat \btheta_k}\}_{k \in S_r}$. Consequently, the server updates the global model by aggregating the locally updated parameters $\btheta_{r+1}^g = \sum_{k \in \l S_r\l} \frac{\l \cD_k \l}{\sum_{k \in \l S_r\l} \l \cD_k \l} {\widehat \btheta_k}$. This process continues for $R$ communication rounds. \\

\noindent\textbf{Knowledge distillation.} Given a dataset of input images, denoted as $\cX$, the goal is to train a student model $\cS$ that approximates the behavior of a teacher model $\cT$.
To facilitate this transfer of knowledge, the knowledge distillation loss is defined as follows:
\begin{align*}
\mathcal{L}_{KD} = \text{KL}\left[\sigma\left(\cT(\cX)\right) \, \Vert \, \sigma\left(\cS(\cX)\right)\right],
\end{align*}
where $\sigma$ represents sotfmax function with temperature $T$ defined as $\sigma(\bz)_i = \frac{\exp(z_i / T)}{\sum_j \exp(z_j / T)}$, and $\text{KL}$ represents the Kullback-Leibler divergence.

\noindent\textbf{Task Arithmetic.} A task $t$ is defined as a specific instance of a dataset paired with a corresponding loss function. For any given task $t$, a task vector is derived by subtracting the model's pre-trained weights $\btheta_{pre}$ from its fine-tuned weights $\btheta_{ft}^t$ on task $t$ , i.e. $\tau_t = \btheta_{ft} - \btheta_{pre}$. To construct a model that performs adeptly across multiple tasks $\{\tau_t\}_{t=1}^{T}$, the task vectors are aggregated and then applied to the pre-trained model weights, resulting in $\btheta = \btheta_{pre} + \lambda \sum_{t=1}^T \tau_t$. Here, $\lambda \in [0,1]$ serves as a hyperparameter that controls the extent of model adaptation. Task arithmetic offers a straightforward, cost-efficient, and scalable method for model editing, demonstrating superior performance compared to methods such as weight averaging.


%Then, the task vectors of multiple tasks $\{\tau_t\}_{t=1}^{T}$ are summed and merged to the pre-trained model, i.e. $\btheta = \btheta_{pre} + \lambda \sum_{t=1}^T \tau_t$, where $\lambda \in [0,1]$ is a hyperparamter denotes the importance of model merging. 

%For multiple tasks ${\tau_t}{t=1}^{T}$, their task vectors are aggregated and then applied to the pre-trained model weights, resulting in $\btheta = \btheta{pre} + \lambda \sum_{t=1}^T \tau_t$, where $\lambda$ is a 

%reflecting the relative importance of each task's contribution to the merged model

%Prior works have mainly focused on solving FL challenges such as data heterogeneity and model heterogeneity for either cross-device or cross-silo environments. In cross-device environment~\cite{yang2019federated, kairouz2021advances}, the clients are typically edge devices with small amount of data and massive amount of clients, while in cross-silo environment~\cite{huang2022cross, kairouz2021advances}, clients are typically powerful entities such as supercomputers with small number of clients and big amount of data.
%However, in real-world several different classes of devices from smartphones to supercomputers can coexist together where each class of device has its own specific model architecture, computation budge, number of users and amount of data. For example, class of smartphones have small computation capability which can train a small model with fewer number of training steps compared to class of supercomputers which can train a large model with bigger number of training steps. Furthermore, class of smartphones has a large number of clients and small amount of data while class of supercomputers has a small number of clients and big dataset size. These coexisting different classes of devices participate in FL to achieve better performance (see Figure 1). To the best of our knowledge we are the first work defining this real-world problem and aim to solve it. Furthermore, our new problem incorporates several challenges of FL, in contrast to prior works trying to solve one challenge at the time.


==> nsecs/backup_experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Same-size device 

\begin{table*}[th]
  \caption{Performance Results on Same-Size Devices. Resnet-20, Resnet-32, ShufflenetV2}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.99\linewidth}{!}{
  \begin{tabular}{ll|llll|llll}
    \toprule
     %\hdottedline{3}{4}{10}
    \multirow{2}{*}{Dataset} & \multicolumn{1}{l|}{\multirow{2}{*}{Baseline}} & \multicolumn{4}{c|}{Low Data Heterogeneity} & \multicolumn{4}{c}{High Data Heterogeneity}\\
    \cmidrule(lr){3-6}
    \cmidrule(lr){7-10}
    & & \multicolumn{1}{c}{Small Device} & \multicolumn{1}{c}{Medium Device} & \multicolumn{1}{c}{Large Device} & \multicolumn{1}{c|}{Average} & \multicolumn{1}{c}{Small Device} & \multicolumn{1}{c}{Small Device} & \multicolumn{1}{c}{Small Device} & \multicolumn{1}{c}{Average}\\
    \midrule
    \multirow{5}{*}{\makecell{CIFAR-10}} & FedAvg & $28.34\pm4.48$\% & $31.35\pm0.95$\% & $28.89\pm2.02$\% & $xx$\% & $15.21\pm2.31$\% & $14.92\pm4.53$\% & $17.62\pm3.95$\% & $xx$\%\\
    & FedDF & $39.33\pm0.56$\% & $41.55\pm2.41$\% & $30.72\pm4.16$\% & $xx$\% & $20.35\pm4.15$\% & $19.22\pm1.87$\% & $17.67\pm4.08$\% & $xx$\%\\
    & FedET & $43.29\pm2.75$\% & $40.44\pm4.20$\% & $33.03\pm2.20$\% & $xx$\% & $24.05\pm2.25$\% & $28.74\pm0.90$\% & $22.06\pm1.18$\% & $xx$\%\\
    & FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\%\\
    & FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\%\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \midrule
    \multirow{5}{*}{\makecell{CIFAR-100}} & FedAvg & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\%\\
    & FedDF & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\%\\
    & FedET & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\%\\
    & FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\%\\
    & FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\%\\
    % \midrule
    % \multirow{6}{*}{\makecell{Reserved}} & FedAvg & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\%\\
    % & FedProx & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\%\\
    % & FedDF & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\%\\
    % & FedET & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\% & $xx$\%\\
    % & FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\%\\
    % & FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\%\\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Scalability for Dir 0.5 and E=20}

\begin{table*}[h]
  \caption{Device Scalability (7): CINIC-10}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.70\linewidth}{!}{
  \begin{tabular}{l|llllllll}
    \toprule
     %\hdottedline{3}{4}{10}
     Baseline & \multicolumn{1}{c}{XXS} & \multicolumn{1}{c}{XS} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{L} & \multicolumn{1}{c}{XL} & \multicolumn{1}{c}{XXL} & \multicolumn{1}{c}{Average}\\
    \midrule
    FedAvg & $21.47\pm0.59$\% & $24.30\pm0.14$\% & $31.47\pm0.02$\% & $35.53\pm0.24$\% & $45.76\pm1.52$\% & $51.78\pm0.14$\% & $59.34\pm0.13$\% & $xx$\%\\
    FedDF & $26.28\pm0.03$\% & $29.990.28$\% & $36.70\pm0.16$\% & $41.71\pm0.38$\% & $52.41\pm0.21$\% & $55.47\pm0.07$\% & $61.72\pm0.05$\% & $xx$\%\\
    FedET & $26.45\pm0.13$\% & $31.32\pm0.22$\% & $38.32\pm0.29$\% & $44.57\pm0.12$\% & $53.83\pm0.10$\% & $56.75\pm0.32$\% & $62.0\pm0.13$\% & $xx$\%\\
    FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}
\begin{table*}[h]
  \caption{Device Scalability (5): CINIC-10}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.60\linewidth}{!}{
  \begin{tabular}{l|llllll}
    \toprule
     %\hdottedline{3}{4}{10}
     Baseline & \multicolumn{1}{c}{XXS} & \multicolumn{1}{c}{XS} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{XL} & \multicolumn{1}{c}{Average}\\
    \midrule
    FedAvg & $21.47\pm0.59$\% & $24.30\pm0.14$\% & $31.47\pm0.02$\% & $35.53\pm0.24$\% & $51.78\pm0.14$\% & $xx$\% \\
    FedDF & $26.10\pm0.25$\% & $29.54\pm0.1$\% & $37.34\pm0.34$\% & $43.03\pm0.17$\% & $53.76\pm1.18$\% & $xx$\% \\
    FedET & $26.75\pm0.17$\% & $30.77\pm0.02$\% & $38.61\pm0.06$\% & $44.83\pm0.03$\% & $56.39\pm0.19$\% & $xx$\% \\
    FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}
\begin{table*}[th]
  \caption{Device Scalability (3): CINIC-10}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.60\linewidth}{!}{
  \begin{tabular}{l|llll}
    \toprule
     %\hdottedline{3}{4}{10}
     Baseline & \multicolumn{1}{c}{XXS} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{Average}\\
    \midrule
    FedAvg & $21.47\pm0.59$\% & $31.47\pm0.02$\% & $35.53\pm0.24$\% & $xx$\% \\
    FedDF & $25.44\pm0.42$\% & $35.75\pm0.06$\% & $41.91\pm0.22$\% & $xx$\% \\
    FedET & $25.06\pm0.17$\% & $36.34\pm0.9$\% & $42.32\pm0.22$\% & $xx$\% \\
    FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    \bottomrule
  \end{tabular}
  }
%\vspace{-20mm}
\end{table*}
%\vspace{-20mm}
\begin{table*}[bh]
  \caption{Device Scalability (2): CINIC-10}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.50\linewidth}{!}{
  \begin{tabular}{l|lll}
    \toprule
     %\hdottedline{3}{4}{10}
     Baseline & \multicolumn{1}{c}{XXS} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{Average}\\
    \midrule
    FedAvg & $21.47\pm0.59$\% & $35.53\pm0.24$\% & $xx$\% \\
    FedDF & $24.39\pm0.89$\% & $39.63\pm0.23$\% & $xx$\% \\
    FedET & $23.74\pm0.88$\% & $41.11\pm0.2$\% & $xx$\% \\
    FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\%\\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}

\subsection{Scalability for Dir 0.3 and E=10}

\begin{table*}[th]
  \caption{Device Scalability (7): CINIC-10 -- Dir 0.3 and E=10}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.70\linewidth}{!}{
  \begin{tabular}{l|llllllll}
    \toprule
     %\hdottedline{3}{4}{10}
     Baseline & \multicolumn{1}{c}{XXS} & \multicolumn{1}{c}{XS} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{L} & \multicolumn{1}{c}{XL} & \multicolumn{1}{c}{XXL} & \multicolumn{1}{c}{Average}\\
    \midrule
    FedAvg & $23.42\pm0.22$\% & $19.45\pm0.52$\% & $26.25\pm0.29$\% & $31.36\pm0.71$\% & $37.38\pm0.01$\% & $41.55\pm0.51$\% & $52.65\pm0.06$\% & $xx$\%\\
    FedDF & $28.47$\% & $27.27$\% & $34.22$\% & $39.66$\% & $44.64$\% & $46.41$\% & $56.31$\% & $xx$\%\\
    FedET & $28.81\pm0.39$\% & $28.71\pm0.29$\% & $34.90\pm0.19$\% & $41.53\pm0.11$\% & $46.44\pm0.22$\% & $48.45\pm0.80$\% & $54.74\pm0.16$\% & $xx$\%\\
    FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}
\begin{table*}[th]
  \caption{Device Scalability (5): CINIC-10, Dir 0.3 and E=10}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.60\linewidth}{!}{
  \begin{tabular}{l|llllll}
    \toprule
     %\hdottedline{3}{4}{10}
     Baseline & \multicolumn{1}{c}{XXS} & \multicolumn{1}{c}{XS} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{XL} & \multicolumn{1}{c}{Average}\\
    \midrule
    FedAvg & $23.42\pm0.22$\% & $19.45\pm0.52$\% & $26.25\pm0.29$\% & $31.36\pm0.71$\% & $41.55\pm0.51$\% & $xx$\% \\
    FedDF & $26.63\pm0.40$\% & $26.75\pm0.87$\% & $32.87\pm0.19$\% & $39.26\pm0.52$\% & $49.84\pm0.79$\% & $xx$\% \\
    FedET & $26.89\pm0.79$\% & $28.44\pm0.11$\% & $33.58\pm0.24$\% & $40.01\pm0.04$\% & $50.83\pm0.15$\% & $xx$\% \\
    FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}
\begin{table*}[th]
  \caption{Device Scalability (3): CINIC-10, Dir 0.3 and E=10}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.60\linewidth}{!}{
  \begin{tabular}{l|llll}
    \toprule
     %\hdottedline{3}{4}{10}
     Baseline & \multicolumn{1}{c}{XXS} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{Average}\\
    \midrule
    FedAvg & $23.42\pm0.22$\% & $26.25\pm0.29$\% & $31.36\pm0.71$\%  & $xx$\% \\
    FedDF & $26.77\pm0.16$\% & $31.59\pm0.08$\% & $37.61\pm0.05$\% & $xx$\% \\
    FedET & $25.53\pm0.63$\% & $31.51\pm0.21$\% & $35.31\pm0.37$\% & $xx$\% \\
    FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}
\begin{table*}[th]
  \caption{Device Scalability (2): CINIC-10, Dir 0.3 and E=10}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.60\linewidth}{!}{
  \begin{tabular}{l|lll}
    \toprule
     %\hdottedline{3}{4}{10}
     Baseline & \multicolumn{1}{c}{XXS} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{Average}\\
    \midrule
    FedAvg & $23.42\pm0.22$\% & $31.36\pm0.71$\% & $xx$\% \\
    FedDF & $25.98\pm0.36$\% & $35.60\pm0.27$\% & $xx$\% \\
    FedET & $25.67\pm0.40$\% & $36.35\pm0.05$\% & $xx$\% \\
    FedHD (w/o SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\% \\
    FedHD (w SG) & $\bf{xx}$\% & $\bf{xx}$\% & $\bf{xx}$\%\\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\begin{table*}[th]
  \caption{Performance Results on Hetero-family.}
  %\vspace{-2mm}
  \label{tab:cifar10}
  \centering
  \aboverulesep = 0.605mm
  \belowrulesep = 0.984mm
  \resizebox{0.99\linewidth}{!}{
  \begin{tabular}{ll|llll|llll}
    \toprule
     %\hdottedline{3}{4}{10}
    \multirow{2}{*}{Dataset} & \multicolumn{1}{l|}{\multirow{2}{*}{Baseline}} & \multicolumn{4}{c|}{Low Data Heterogeneity} & \multicolumn{4}{c}{High Data Heterogeneity}\\
    \cmidrule(lr){3-6}
    \cmidrule(lr){7-10}
    & & \multicolumn{1}{c}{Small Device} & \multicolumn{1}{c}{Medium Device} & \multicolumn{1}{c}{Large Device} & \multicolumn{1}{c|}{Average} & \multicolumn{1}{c}{Small Device} & \multicolumn{1}{c}{Medium Device} & \multicolumn{1}{c}{Large Device} & \multicolumn{1}{c}{Average}\\
    \midrule
    \multirow{6}{*}{\makecell{CIFAR-10}} & FedAvg & $27.53\pm0.83$\% & $47.30\pm3.17$\% & $55.10\pm8.60$\% & $xx$\% & $20.93\pm1.54$\% & $25.62\pm6.04$\% & $36.80\pm5.47$\% & $xx$\%\\
    %& FedProx & $29.42\pm0.61$\% & $52.39\pm1.97$\% & $69.54\pm4.66$\% & $xx$\% & $19.85\pm1.08$\% & $28.80\pm3.04$\% & $45.40\pm6.17$\% & $xx$\%\\
    & FedDF & $34.15\pm0.87$\% & $54.06\pm1.06$\% & $69.07\pm4.99$\% & $xx$\% & $24.20\pm0.74$\% & $34.07\pm3.08$\% & $39.81\pm5.45$\% & $xx$\%\\
    & FedET & $33.24\pm1.27$\% & $58.86\pm0.94$\% & $65.56\pm3.49$\% & $xx$\% & $26.37\pm1.26$\% & $40.77\pm4.71$\% & $43.64\pm3.36$\% & $xx$\%\\
    & FedHD (w/o SG) & $\bf{33.29\pm0.15}$\% & $\bf{57.64\pm0.19}$\% & $\bf{68.44\pm0.66}$\% & $\bf{xx}$\% & $\bf{24.92\pm1.32}$\% & $\bf{38.07\pm3.19}$\% & $\bf{48.01\pm3.99}$\% & $\bf{xx}$\%\\
    & FedHD (w SG) & $\bf{33.34\pm3.36}$\% & $\bf{58.01\pm3.12}$\% & $\bf{70.22\pm4.40}$\% & $\bf{xx}$\% & $\bf{25.10\pm1.87}$\% & $\bf{38.81\pm5.36}$\% & $\bf{50.26\pm6.42}$\% & $\bf{xx}$\%\\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \midrule
    \multirow{6}{*}{\makecell{CIFAR-100}} & FedAvg & $8.51\pm0.37$\% & $22.11\pm0.58$\% & $37.91\pm2.60$\% & $xx$\% & $7.01\pm0.47$\% & $14.94\pm0.96$\% & $28.51\pm1.46$\% & $xx$\%\\
    %& FedProx & $8.66\pm0.22$\% & $23.37\pm0.35$\% & $36.60\pm0.11$\% & $xx$\% & $6.73\pm0.28$\% & $17.86\pm0.16$\% & $31.74\pm0.53$\% & $xx$\%\\
    & FedDF & $10.46\pm0.17$\% & $23.46\pm0.65$\% & $36.81\pm0.82$\% & $xx$\% & $7.76\pm0.4$\% & $18.92\pm0.39$\% & $29.81\pm1.09$\% & $xx$\%\\
    & FedET & $11.16\pm0.18$\% & $25.40\pm0.30$\% & $37.38\pm0.60$\% & $xx$\% & $8.20\pm0.54$\% & $20.66\pm0.50$\% & $28.95\pm1.79$\% & $xx$\%\\
    & FedHD (w/o SG) & $\bf{10.29\pm0.11}$\% & $\bf{27.14\pm0.89}$\% & $\bf{39.15\pm0.88}$\% & $\bf{xx}$\% & $\bf{7.88\pm0.68}$\% & $\bf{21.41\pm0.37}$\% & $\bf{31.31\pm0.66}$\% & $\bf{xx}$\%\\    
    & FedHD (w SG) & $\bf{11.25\pm0.37}$\% & $\bf{27.86\pm0.86}$\% & $\bf{38.68\pm0.45}$\% & $\bf{xx}$\% & $\bf{8.45\pm0.20}$\% & $\bf{22.16\pm0.87}$\% & $\bf{31.95\pm1.13}$\% & $\bf{xx}$\%\\
    \bottomrule
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table*}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> nsecs/empirical_study.tex <==
\section{Empirical Study}
We first conduct a thorough empirical study on various factors affecting clusters of heterogeneous devices setting in FL. For simplicity, we use a setting of 2 clusters, 20 clients for each cluster, client sample rate 0.4 for both cluster and private data is cifar10 and public dataset is cifar100. We set the local epochs to 20, batch size to 10 and communication rounds to 50 for both clusters. We consider three baselines: FedAvg, FedDF, FedET. FedAvg is a simple baseline which perform per-cluster FL and there is no knowledge transfer from other clusters. This is used as a baseline to evaluate how the knoweldge transfer has helped to improve models in device heterogenous baselines.

\textbf{Effect of Dataset Ratios.} Table 1 shows the result.

\begin{table}[h]
    \centering
    \caption{Homo Family: ResNet-8 and ResNet-18}
    \label{tab:my_label}
    \resizebox{0.70\linewidth}{!}{
    \begin{tabular}{ll|lll}
    \toprule
    Architecture Setting & Baseline & Small Devices & Large Devices & Average \\
    \midrule
    \multicolumn{5}{c}{Data Split: 50\% -- 50\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Homo-Family\\(ResNet)}}  &  FedAvg & $54.96\pm5.44$ & $58.96\pm2.01$ & $56.96$\\
     & FedDF(SOLO) & $59.02\pm1.55$ & $57.05\pm0.21$ & $58.03$ \\
      & FedDF(AvgKD) & $61.51\pm2.31$ & $62.12\pm0.72$ & $61.81$ \\
    & FedDF(fixed) & $54.88\pm2.61$ & $57.28\pm0.54$ & $56.08$ \\
         %& FedET & xx & xx & xx \\
     % \midrule
     % \multirow{3}{*}{\makecell{Homo-Family\\(VGG)}} & FedAvg & $53.56\pm4.64$ & $49.55\pm0.41$ & $51.55$\\
     %     & FedDF & $53.08$ & $44.03$ & $48.55$ \\
     %     & FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 30\% -- 70\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Homo-Family\\(ResNet)}}  &  FedAvg & $54.29\pm0.23$ & $64.46\pm2.58$ & $59.37$\\
     & FedDF(SOLO) & $51.47\pm2.39$ & $62.19\pm1.62$ & $56.83$ \\
    & FedDF(AvgKD) & $57.19\pm2.37$ & $63.23\pm1.95$ & $60.21$ \\
    & FedDF(Fixed) & $54.44\pm1.67$ & $61.68\pm1.58$ & $58.06$ \\
         %& FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 10\% -- 90\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Homo-Family\\(ResNet)}}  &  FedAvg & $42.99\pm0.84$ & $66.19\pm0.22$ & $54.59$\\
     & FedDF(SOLO) & $40.33\pm3.03$ & $62.98\pm0.47$ & $51.65$ \\
    & FedDF(AvgKD) & $48.69\pm0.47$ & $62.03\pm0.76$ & $55.36$ \\
    & FedDF(Fixed) & $47.99\pm1.28$ & $62.51\pm0.46$ & $55.25$ \\
        % & FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 70\% -- 30\%} \\
    \midrule
      \multirow{2}{*}{\makecell{Homo-Family\\(ResNet)}}  &  FedAvg & xx & xx & xx\\
         & FedDF & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 90\% -- 10\%} \\
    \midrule
      \multirow{2}{*}{\makecell{Homo-Family\\(ResNet)}}  &  FedAvg & xx & xx & xx\\
         & FedDF & xx & xx & xx \\
     \bottomrule
    \end{tabular}
    }
\end{table}

\begin{table}[h]
    \centering
    \caption{Hetero Family Arch: ResNet-8 and VGG-16}
    \resizebox{0.70\linewidth}{!}{
    \begin{tabular}{ll|lll}
    \toprule
    Architecture Setting & Baseline & Small Devices & Large Devices & Average \\
    \midrule
    \multicolumn{5}{c}{Data Split: 50\% -- 50\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Hetero-Family\\(ResNet-8 VGG-16)}}  &  FedAvg & $54.96\pm5.44$ & $53.97\pm5.66$ & $54.46$\\
     & FedDF(SOLO) & $58.73\pm1.68$ & $45.29\pm1.93$ & $52.01$ \\
      & FedDF(AvgKD) & $52.24\pm2.45$ & $45.90\pm2.11$ & $49.07$ \\
    & FedDF(fixed) & $42.32\pm1.39$ & $45.60\pm0.48$ & $43.96$ \\
         %& FedET & xx & xx & xx \\
     % \midrule
     % \multirow{3}{*}{\makecell{Homo-Family\\(VGG)}} & FedAvg & $53.56\pm4.64$ & $49.55\pm0.41$ & $51.55$\\
     %     & FedDF & $53.08$ & $44.03$ & $48.55$ \\
     %     & FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 30\% -- 70\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Hetero-Family\\(ResNet-8 VGG-16)}}  &  FedAvg & $54.29\pm0.23$ & $58.65\pm1.08$ & $56.47$\\
     & FedDF(SOLO) & $51.11\pm2.03$ & $55.34\pm3.81$ & $53.22$ \\
    & FedDF(AvgKD) & $51.90\pm2.98$ & $57.33\pm2.60$ & $54.61$ \\
    & FedDF(Fixed) & $45.46\pm1.94$ & $56.89\pm4.08$ & $51.17$ \\
         %& FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 10\% -- 90\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Hetero-Family\\(ResNet-8 VGG-16)}}  &  FedAvg & $42.99\pm0.84$ & $61.30\pm4.11$ & $52.14$\\
     & FedDF(SOLO) & $39.09\pm3.25$ & $54.16\pm2.78$ & $46.62$ \\
    & FedDF(AvgKD) & $44.01\pm0.74$ & $58.21\pm2.67$ & $51.11$ \\
    & FedDF(Fixed) & $40.67\pm0.60$ & $56.28\pm0.36$ & $48.47$ \\
        % & FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 70\% -- 30\%} \\
    \midrule
      \multirow{2}{*}{\makecell{Hetero-Family\\(ResNet-8 VGG-16)}}  &  FedAvg & xx & xx & xx\\
         & FedDF & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 90\% -- 10\%} \\
    \midrule
      \multirow{2}{*}{\makecell{Hetero-Family\\(ResNet-8 VGG-16)}}  &  FedAvg & xx & xx & xx\\
         & FedDF & xx & xx & xx \\
     \bottomrule
    \end{tabular}
    }
    \label{tab:my_label}
\end{table}

\begin{table}[h]
    \centering
    \caption{Hetero Family Arch: ViT-S and ResNet-18}
    \resizebox{0.70\linewidth}{!}{
    \begin{tabular}{ll|lll}
    \toprule
    Architecture Setting & Baseline & Small Devices & Large Devices & Average \\
    \midrule
    \multicolumn{5}{c}{Data Split: 50\% -- 50\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Hetero-Family\\(ViT-S ResNet-18)}}  &  FedAvg & $39.76\pm3.64$ & $58.95\pm2.19$ & $49.35$\\
     & FedDF(SOLO) & $43.52\pm0.68$ & $57.22\pm0.11$ & $50.37$ \\
      & FedDF(AvgKD) & $44.75\pm1.68$ & $60.10\pm0.45$ & $52.42$ \\
    & FedDF(fixed) & $40.51\pm1.58$ & $56.71\pm0.04$ & $48.61$ \\
         %& FedET & xx & xx & xx \\
     % \midrule
     % \multirow{3}{*}{\makecell{Homo-Family\\(VGG)}} & FedAvg & $53.56\pm4.64$ & $49.55\pm0.41$ & $51.55$\\
     %     & FedDF & $53.08$ & $44.03$ & $48.55$ \\
     %     & FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 30\% -- 70\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Hetero-Family\\(ViT-S ResNet-18)}}  &  FedAvg & $41.02\pm1.45$ & $61.42\pm0.47$ & $51.22$\\
     & FedDF(SOLO) & $41.02\pm1.32$ & $61.15\pm1.27$ & $51.08$ \\
    & FedDF(AvgKD) & $42.32\pm0.25$ & $62.99\pm1.44$ & $52.65$ \\
    & FedDF(Fixed) & $39.32\pm0.71$ & $61.31\pm0.98$ & $50.31$ \\
         %& FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 10\% -- 90\%} \\
    \midrule
      \multirow{3}{*}{\makecell{Hetero-Family\\(ViT-S ResNet-18)}}  &  FedAvg & $31.57\pm1.28$ & $64.45\pm1.97$ & $48.01$\\
     & FedDF(SOLO) & $33.59\pm0.77$ & $63.31\pm0.49$ & $48.45$ \\
    & FedDF(AvgKD) & $36.30\pm0.04$ & $64.05\pm0.24$ & $50.17$ \\
    & FedDF(Fixed) & $34.50\pm0.05$ & $63.45\pm0.24$ & $48.97$ \\
        % & FedET & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 70\% -- 30\%} \\
    \midrule
      \multirow{2}{*}{\makecell{Hetero-Family\\(ViT-S ResNet-18)}}  &  FedAvg & xx & xx & xx\\
         & FedDF & xx & xx & xx \\
     \midrule
    \multicolumn{5}{c}{Data Split: 90\% -- 10\%} \\
    \midrule
      \multirow{2}{*}{\makecell{Hetero-Family\\(ViT-S ResNet-18)}}  &  FedAvg & xx & xx & xx\\
         & FedDF & xx & xx & xx \\
     \bottomrule
    \end{tabular}
    }
    \label{tab:my_label}
\end{table}

\begin{table}[h]
    \centering
    \caption{Effect of Different Public datasets}
    \resizebox{0.70\linewidth}{!}{
    \begin{tabular}{ll|lll}
    \toprule
    Baseline & Public Dataset & Small Devices & Large Devices & Average \\
    \midrule
    FedAvg & -- & $54.96\pm5.44$ & $58.96\pm2.01$ & $56.96$\\
    \midrule
    FedDF(AvgKD) & CIFAR-100 (0.99) & $61.51\pm2.31$ & $62.12\pm0.72$ & $61.81$ \\
    FedDF(AvgKD) & TinyImagenet (0.92) & $51.69\pm0.43$ & $49.54\pm0.37$ & $50.61$ \\
    FedDF(AvgKD) & Caltech-256 (0.89) & $51.71\pm0.44$ & $48.84\pm0.52$ & $50.27$ \\
    FedDF(AvgKD) & GTSRB (0.85) & $49.14\pm0.11$ & $49.73\pm0.81$ & $49.43$ \\
    FedDF(AvgKD) & Celeb-A (0.77) & $45.02\pm1.40$ & $45.12\pm1.62$ & $45.07$ \\
    FedDF(AvgKD) & Food-101 (0.65) & $51.54\pm1.56$ & $49.70\pm3.05$ & $50.62$ \\
     \bottomrule
    \end{tabular}
    }
    \label{tab:my_label}
\end{table}

==> nsecs/intro.tex <==
\section{Introduction}

\begin{figure}[ht]
    \centering
     \includegraphics[width=.99\linewidth]{figs/problem.png}
     \vspace{-8mm}
    \caption{\textbf{Clusters of Heterogeneous Devices.} This figure provides an overview of the clusters of heterogeneous devices problem in a scenario with three clusters: small devices (smartphones), medium devices (computers), and large devices (supercomputers). Heterogeneous devices, each with its specific configuration, actively participate in FL to collectively train their unique global model architecture.}
    \label{fig:problem}
    \vspace{-4mm}
\end{figure} 

The proliferation of edge devices, such as IoT devices and smartphones, has propelled them into becoming primary platforms for computing and machine learning tasks. These devices host vast and diverse datasets, which are invaluable for enhancing machine learning models. Yet, the sharing of their local data raises significant privacy concerns among client. To address these privacy concerns, federated learning (FL) has emerged as a promising distributed machine learning training framework without requiring data sharing. %FL enables training of a shared global model collaboration with multiple clients without requiring data sharing.
Despite its success, the existing FL methods lack support for device heterogeneous settings.
However, the majority of existing works mainly focus on the unrealistic \emph{model-homogeneous} setting where all clients are assumed to have the same computation power and can train an identical machine learning model~\cite{li2020federated, mcmahan2017communication, wang2020tackling, karimireddy2020scaffold, li2021model, wang2020federated, liu2022deep}.

Federated Learning (FL) has emerged as a promising decentralized machine learning framework without requiring raw data sharing.

Federated Learning (FL) has received lots attention recently, due to its success in training machine learning models in collaboration of multiple devices without requiring direct data sharing; thus enhancing privacy of users. Yet, the majority of existing works predominantly focus on the unrealistic \emph{device-homogeneous} setting where all device prototypes are assumed to be identical and training an identical neural network architecture~\cite{li2020federated, mcmahan2017communication, wang2020tackling, karimireddy2020scaffold, li2021model, wang2020federated, liu2022deep}. This concentration (assumption) excludes the participation of \emph{heterogeneous devices}, each possessing its unique and unhashable neural network architecture, all of which can significantly enhance the model performance due to their unique and invaluable data.

To enhance the potentials of FL and include heterogeneous device prototypes into the federation, researchers have proposed partial model training (PT) technique recently. In PT-based approach, clients are tasked with training sub-models extracted from the global model based on their computational capabilities~\cite{diao2020heterofl, alam2022fedrolex, horvath2021fjord}. However, this approach require the participant device prototypes accommodate different model architectures which may not be optimal according to their machine learning task and specific hardware and software system. In real-world, each device has its own distinct and unhashable model architecture designed to align its specific hardware and software system as well as machine learning task and may not accommodate different model architectures. To address this issue and have a more practical device heterogeneous FL setting, knowledge distillation (KD) techniques has been proposed. In KD-based approach, server utilizes a public dataset to transfer knowledge across heterogeneous device prototypes with heterogeneous model architecture. Specifically, FedDF~\cite{lin2020ensemble}, propose averaged ensemble distillation on an unlabeled public dataset. 
%perform knowledge distillation using averaged ensembles' logits on an unlabeled public dataset. 
FedET, propose a confidence-based weighted ensemble distillation with a diversity regularization to better handle presence of data heterogeneity. However, these prior works have considered same-size device prototypes with same-size dataset and models. In practice, device prototypes vary significantly in their size including dataset and model.

In this paper we revisit KD-based approaches and conduct a thorough experimental study. We observe two major limitations. (1) The existing KD-based methods do not scale to different size devices including small devices with small model architecture and dataset up to the other end of spectrum with large devices with large model architecture. We notice that as device prototypes become larger the existing KD-based methods only enhance the performance of small devices while hurting the large ones. (2) The existing KD-based methods rely on a very similar public dataset to the local private dataset which may not be practical as server does not have any knowledge about the local private dataset and are not robust to more different public datasets. Interestingly, in our empirical study we observe that using a less similar public dataset can significantly drop the performance of the existing KD-based methods.

Therefore, there is an increasing need to developed FL methods where different size device prototypes with different model architecture and dataset size can enhance their performance. Furthermore, as the world is moving towards larger devices with larger model architectures and dataset sizes, this need becomes more significant.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Federated Learning (FL) is a distributed machine learning paradigm where multiple clients collaboratively train a shared global model under the orchestration of a central server, while preserving the privacy of clients' local data~\cite{mcmahan2017communication, Peter-Kairouz2021}. Although FL has shown promising results in The majority of existing works mainly focus on the unrealistic \emph{model-homogeneous} setting where all clients are assumed to have the same computation power and can train an identical machine learning model~\cite{li2020federated, mcmahan2017communication, wang2020tackling, karimireddy2020scaffold, li2021model, wang2020federated, liu2022deep}. In pursuit of a more practical setup, several efforts have been made to develop \emph{model-heterogeneous} FL algorithms, where the goal is to enable clients to train heterogeneous models based on their computational capabilities. These works either propose knowledge distillation (KD)~\cite{hinton2015distilling} techniques to train a larger~\cite{cho2022heterogeneous} or multiple global models~\cite{lin2020ensemble, sattler2021fedaux} at the server using the logits of various-sized ensembles on a public dataset or introduce  partial model training (PT) techniques. In PT-based approach, clients are tasked with training sub-models extracted from the global model based on their computational capabilities~\cite{diao2020heterofl, alam2022fedrolex, horvath2021fjord}.

However, in reality there exists a diverse spectrum of device classes, including IoT devices, smartphones, desktop computers, and supercomputers, each class with distinctive computational power, memory capacities, and unhashable model architectures designed to align their specific hardware and software systems (\textbf{device heterogeneity}). Consequently, it is natural to contemplate a federated learning setting where heterogeneous device classes, each employing varying model architectures, join forces to learn from one another. Furthermore, other FL configurations such as the number of clients, training budget, and dataset size for each device class may vary significantly. For instance, smartphones (a cluster of small devices) typically feature a larger number of clients, constrained local training budgets, smaller model sizes, limited availability, and smaller local datasets in comparison to supercomputers (a cluster of large devices). Supercomputers, on the other hand, generally have fewer clients, substantial training budgets, larger model sizes, consistent availability, and extensive local datasets. Additionally, recent studies have highlighted the immense capabilities of large models~\cite{bommasani2021opportunities, wei2022emergent, kaplan2020scaling}. Therefore, as the demand for devices capable of accommodating large models continues to grow, there is an increasing need to develop advanced FL algorithms that can facilitate collaboration among devices ranging from small to large.

In this paper, we take a substantial step forward by introducing a new multifaceted real-world FL problem, which we term the \textbf{``clusters of heterogeneous devices''}. We consider a federated learning problem where diverse clusters of heterogeneous devices, ranging from small to large, each equipped with distinct models, memory capacities, and computational resources, collaborate to enhance each other's global model. In this problem, each cluster may have different FL configurations, including number of clients, training budgets, dataset sizes, and even potentially different FL optimizers. Figure~\ref{fig:problem} provides a visual representation of this problem. 
%The introduced problem differs from the model-heterogeneous setting in FL in three significant ways: (1) each device cluster may operate with distinct FL configurations and optimizers, (2) unlike prior works~\cite{diao2020heterofl, alam2022fedrolex, horvath2021fjord} that assume clients can train heterogeneous models assigned to them by the server, here, clients are allowed to have their unique, unhashable architectures, (3) this problem not only addresses the challenge of model-heterogeneity but also encompasses other challenges such as data heterogeneity and system heterogeneity.

Furthermore, we propose a novel knowledge distillation (KD)-based framework, \textbf{FedHD} (\textbf{Fed}erated Learning for \textbf{H}eterogeneous \textbf{D}evices), embracing clusters of heterogeneous devices in FL. In our approach, heterogeneous ensembles (clients models) serve as teachers to transfer their knowledge into the global models of the clusters serving as the students using a public unlabeled dataset at the server. For each cluster's global model server-side training, FedHD combines heterogeneous ensemble distillation objectives using an adaptive weighting scheme based on the model sizes of the ensembles. The fundamental intuition behind the adaptive weighting scheme is that smaller models can benefit more from larger models, while smaller models are less beneficial for larger models. Additionally, the presence of domain differences between the public dataset and the local private dataset introduces noise and unreliability in the ensembles' logits on the public dataset. This may negatively impact the ensemble distillation process and drift the global models into erroneous directions. To address this potential issue, we design a self-gaurded regularization term which protects each cluster's global model by preserving the its initial logits on the public dataset during the ensemble distillation process. We empirically evaluate the performance of FedHD in two different architecture settings: (1) ``homo-family,'' where clusters' models belong to the same architecture family (e.g., different-sized ResNets), and (2) ``hetero-family,'' where clusters' models may not necessarily belong to the same architecture family. Our experiments demonstrate that FedHD achieves state-of-the-art performance results in both settings on CIFAR-10 and CIFAR-100 datasets, showcasing its efficacy in addressing the introduced new problem. \\

\noindent\textbf{Contributions.} In summary, our paper make the following key contributions:
\begin{itemize}
    \item To the best of our knowledge, we are the first work that define the clusters of heterogeneous devices problem, where each cluster possess a distinct model architecture, memory capacity, dataset size, and FL configurations.
    \item  We propose FedHD, a novel KD-based framework harnessing an adaptively weighted heterogeneous ensemble distillation technique with self-gaurded regularization to address this problem.
    \item Our experimental results show that FedHD consistently achieves state-of-the-art results on various datasets and architectures. \\
\end{itemize}

\noindent\textbf{Organization.} The reset of the paper is organized as follows. In Section~\ref{sec:related_works} we discuss related works. In Section~\ref{sec:problem} we bring the background and problem definition. In Section~\ref{sec:method} we detail our proposed method. In Section~\ref{sec:exp}, we provide the experimental results. In Section~\ref{sec:conclude} we conclude our paper.

==> nsecs/intro_progress.tex <==
\section{Introduction}
\vspace{-0.1in}
Federated Learning (FL) has rapidly gained traction as a promising approach to train machine learning models collaboratively across multiple devices, while preserving the privacy of user data. This is realized by sharing model weights instead of raw data, effectively bypassing the need for direct data sharing. However, the predominant focus of existing research has been on an idealized~\emph{device-homogeneous} setting, wherein all participating devices are assumed to possess identical capabilities and train the same neural network architecture~\cite{li2020federated, mcmahan2017communication, wang2020tackling, karimireddy2020scaffold, li2021model, wang2020federated, liu2022deep}. This assumption overlooks the rich diversity of~\emph{heterogeneous devices} in real-world applications, each with its unique hardware and software configurations and, consequently, its unique neural network architecture. Therefore, including heterogeneous devices in FL is crucial, as each device prototype can significantly enhance the model performance due to its unique and invaluable data.

To enable device heterogeneous FL, recent studies have explored strategies such as partial model training (PT), where clients are assigned sub-models from a global model that align with their computational capabilities~\cite{diao2020heterofl, alam2022fedrolex, horvath2021fjord}. However, these methods often require devices to support different model architectures, which may not align with their underlying machine learning tasks or their specific hardware and software systems. In response to these challenges, knowledge distillation (KD) techniques have been proposed to facilitate knowledge transfer across devices with varying architectures. Specifically, FedDF~\cite{lin2020ensemble} proposes average ensemble distillation using an unlabeled public dataset and FedET introduces a confidence-based weighted ensemble distillation with diversity regularization to better handle the presence of data heterogeneity.~\ul{Despite these advancements, prior works have largely considered same-size device prototypes with same-size dataset and models in their experimentation, a presumption that does not hold in the heterogeneous landscapes of real-world applications, where device capabilities can range widely.}

Current ensemble distillation methods, such as FedDF and Fed-ET, typically focus on same-size devices and do not fully address the challenges of knowledge transfer in settings with device heterogeneity. In practice, devices vary significantly in size and learning capacities, ranging from small devices like IoTs and smartwatches to larger systems such as servers and high-performance workstations.

In this paper, we critically examine KD-based approaches in the context of device heterogeneity within FL. Through comprehensive experimentation, we identify two principal limitations of existing methods: (1) They do not scale well to federation amongst devices of varying sizes, from small devices with small models and datasets to large ones with large models and datasets. We observe that current KD-based methods may enhance the performance of smaller devices, but they detrimentally affect the performance of larger devices. (2) The effectiveness of existing KD-based methods heavily depends on the use of public datasets closely resembling the local private datasets which is impractical as the server typically lacks direct knowledge of the private local datasets. Our findings reveal a notable decline in performance when public datasets less similar to the private local datasets are employed, highlighting the fragility of current approaches. Given these observations, there is a pressing need for FL algorithms that can embrace diverse and heterogeneous devices varying in size, model architecture and dataset volumes. This need is further amplified by the ongoing trend towards larger devices with larger models and datasets.

Recently, task arithmetic technique has appeared as a promising technique in editing the knowledge of pre-trained models. 

\begin{itemize}
    \item Standard FL excludes participation of heterogeneous devices, all of which may contribute to model training due to their unique and invaluable local datasets
    \item Prior works attempt to resolve this issue in two ways: PT-based and KD-based approach
    \item PT-based approach is not practical as in real-world devices may have their unique neural network architecture according to their specific hardware and software system design.
    \item KD-based methods only experiment with same-size devices with same model and dataset size and mainly propose AvgLogits process.
    \item FedDF proposes AvgLogits which has 2 limitations:
    \item FedET propose confidence-based weighted ensemble distillation which again has the same problems as AvgLogits plus x, y
    \item To resolve these issues we proposed FedHD.
    \item To control the importance of each teacher ensemble in the distillation process we consider each ensemble distillation as separate task.
    \item To scaffold the student from negative impact of noisy distillation due insufficient training, lack of similar public data and presence of data heterogeneity we introduce self-guard regularization term into the ensemble distillation tasks.
    \item Rather than considering expensive join-training of different ensemble distillation tasks, which has issues such as gradient conflicts, difficulty in optimization and hyper-parameter tuning, scalability issues, we take an alternative approach
    \item Inspired by recent advances in model editing via task arithmetic, we fine-tune each task separately and merge them using task arithmetic operation.
    \item We further support our study by a providing a theoretical framework why KD is effective in device heterogeneous FL, and further convergence analysis of our method.
    \item We design new experimental cases and show our method works very well.
    \item In the contribution, we list that we formalize the device heterogeneous FL problem, and provide a more comprehensive experimental study with CNN and ViTs.
\end{itemize}

\begin{figure}
    \centering
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=0.75\linewidth]{nfigs/problem_a.png}
        \caption{Device Heterogeneous FL}
        \label{fig:sub1}
    \end{subfigure}
    \hspace{0.03\textwidth}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{nfigs/problem_b.png}
        \caption{AvgLogits}
        \label{fig:sub2}
    \end{subfigure}
    \hspace{0.008\textwidth}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{nfigs/problem_c.png}
        \caption{Our Approach}
        \label{fig:sub3}
    \end{subfigure}
    \caption{\textbf{Distinction of our approach.} (a) shows an overview of device heterogeneous FL where heterogeneous device prototypes with their unique configuration participate in FL. (b) prior works usually ignore that fact that heterogeneous  ensembles may vary in strength and helpfulness significantly and average all logits. (c) in our approach we consider each ensemble distillation as a task and edit the student model with task arithmetic.}
    \label{fig:main}
\end{figure}

%Task arithmetic introduces the notion of a “task vector”, which can be described as a vector of weights fine-tuned specifically for a given task, subtracted from the corresponding pre-trained weights (as illustrated in Fig. 2(a)). Essentially, a task vector serves as a unique representation for a particular task

% Task arithmetic is a powerful techinque in making models capabale of perfoming good on multiple tasks.

%In this work, we a novel FL method called \textbf{FedHD} (\textbf{Fed}erated Learning for \textbf{H}eterogeneous \textbf{D}evices), to addresses the aforementioned major limitations in the existing device heterogeneous KD-based methods. FedHD is based on


% A lack of scalability
%not only accommodate, but also leverage the diversity in device sizes, model architectures, and dataset volumes

 %The effectiveness of existing KD-based methods heavily depends on the use of public datasets closely resembling the local private datasets, a condition that proves impractical given servers typically have no direct insight into these local datasets. Our findings reveal a notable decline in performance when public datasets less similar to the private datasets are employed, emphasizing the brittleness of these approaches. 

%Existing KD-based methods perform optimally only when the public dataset closely resembles the local private dataset. Our studies reveal a significant performance drop when utilizing public datasets that diverge from the private datasets, underscoring the fragility of current approaches. Relying on closely similar public datasets to the local private dataset is impractical, as the server typically lacks direct knowledge of these local datasets. Given these observations, there is a pressing need for FL algorithms that can embrace and leverage the diversity and heterogeneity of devices, varying in size, model architecture, and dataset volumes. This necessity is accentuated by the trend towards larger devices with more complex models and datasets.

==> nsecs/intro_short.tex <==
\section{Introduction}
\vspace{-0.1in}
Federated Learning (FL) has rapidly gained traction as a promising approach to train machine learning models collaboratively across multiple devices, while preserving the privacy of user data. Standard federated learning methods, such as FedAvg~\cite{mcmahan2017communication}, however, are primarily designed for unrealistic~\emph{device-homogeneous} scenarios, where all devices are assumed to have identical compute resource and can train the same neural network architecture~\cite{li2020federated, mcmahan2017communication, wang2020tackling, karimireddy2020scaffold, li2021model, wang2020federated, liu2022deep}. Therefore, standard FL cannot support the participation of \emph{heterogeneous devices}, all of which could significantly contribute to model training due to their unique and invaluable local datasets. 

To address this gap, some studies proposed partial model training techniques. Here, clients are tasked with training specific sub-models extracted from the global model that align with their computational capabilities~\cite{diao2020heterofl, alam2022fedrolex, horvath2021fjord}. Nonetheless, these approaches still face practical, as diverse device prototypes, such as IoT devices and smartphones, often have their own unique unhashable neural network architectures designed for their hardware and software configurations, and underlying machine learning task. Therefore, they may not support training varying model architectures. In response to this limitation, other studies have proposed knowledge distillation techniques to enable federation between heterogeneous device prototypes. Here, locally updated client models of different device prototypes, collectively termed ensembles, serve as teachers to distill their knowledge into each device prototype's server student model using an unlabeled public dataset.

Despite these advancements, current knowledge distillation (KD)-based methods in device heterogeneous FL are primarily designed for scenarios involving same-size device prototypes with similar capabilities and architectures. However, these methods fall short in establishing effective knowledge transfer when applied to real-world settings where device prototypes span a broad range of sizes and capabilities, from small IoT devices to large workstations. This shortfall arises primarily due two reasons: 
(1) Existing methods often disregard the individual strengths and information quality of each device prototype's ensembles and merge their logits into a single distillation target. This approach dilutes the richer, more informative logits from more capable devices with less informative outputs from less capable ones.
(2) Additionally, these methods use this single integrated distillation target to transfer knowledge across all student models, regardless of their size. This one-size-fits-all approach does not account for the differences in architecture and learning capacities among the device prototypes' student models.

% In practice there is a diverse range of devices from small ones like IoTs with small model and small dataset to large ones like workstations with large model and large dataset. These methods fall short in establishing effective knowledge transfer under this challenging real-world settings. 
In this paper, we introduce FedHD, a novel knowledge transfer and integration framework, aimed at addressing the critical limitations in existing methods and enhancing knowledge transfer in scenarios where device capabilities vary. Unlike previous methods that integrate the logits of all heterogeneous ensembles and distill them into every student model, FedHD treats the knowledge transfer from each device prototype's ensembles as separate tasks and distills them independently. This approach ensures that the distinctive knowledge of each device is accurately distilled, without being diluted or altered by logits from other devices. 
Furthermore, to merge the distilled knowledge from each device prototype's ensembles, we propose a novel knowledge integration technique via task arithmetic. In this context, a task vector is defined by subtracting the distilled student model parameters by a specific knowledge transfer task from its initial pre-trained parameters, i.e., the averaged locally updated parameters. Essentially, this task vector serves as a unique representation for the distilled knowledge of a specific device prototype's ensembles. 
To effectively integrate the distilled knowledge from heterogeneous device prototypes' ensembles into the student model, we introduce an adaptive task arithmetic operation. Here, the merging coefficients of each knowledge transfer task determine the amount of knowledge integration from that device prototype's ensembles, allowing the student model to strategically customize the knowledge integration process based on the helpfulness of each device prototype's ensembles and its own learning capacity to achieve maximum performance. Overall, FedHD presents a more effective knowledge transfer and integration, addressing critical limitations in existing methods.

Moreover, the ensemble distillation process can inadvertently lead student models into erroneous directions, causing them to forget the knowledge they acquired through locally updated parameters. This issue arises due to two reasons: 
(1) The distillation process introduces noise, as the ensembles' logits are inferred on an unfamiliar public dataset, distinct from their original training data. Additionally, the presence of data heterogeneity and the insufficient training of some ensembles due to computational constraints can exacerbate this noise. (2) the distillation lacks supervision from the actual private datasets, which are the ultimate learning objectives. 
To scaffold the student models from the unsupervised and noisy distillation process, which may cause them to drift in erroneous directions and forget their acquired knowledge, we introduce a self-regularization technique into the knowledge transfer process from each device prototype's ensembles. Our self-regularization technique mitigates these issues by enforcing similarity between the logits of the student model and its initial logits, thus stabilizing the learning process.

We further support our algorithm with convergence results, and comprehensive empirical evaluation. 

The contribution of our paper is as follow:
\begin{itemize}
    \item We formalize the problem of federated learning with heterogeneous device prototypes
    \item We propose a novel knowledge transfer and integration method, called FedHD, which addresses the fundamental limitations of prior works in device heterogeneous scenarios where device prototypes sizes and capabilities vary.
    \item We support our algorithm by convergence analysis
    \item We provide comprehensive empirical evaluations.
\end{itemize}

\begin{comment}

As a result, the richer, more informative logits from more capable devices are diluted by less informative outputs from less capable devices. This single integrated distillation target does not fully exploit the unique contributions of more accurate models and could potentially degrade the overall quality of the knowledge being transferred. 

Furthermore, they use this single integrated distillation target for knowledge transfer all different size student models.
This one-size-fits-all approach overlooks the difference in the architecture and learning capacities between device prototypes' student models and lack to customize knowledge transfer. Therefore, effectiveness of knowledge transfer in existing method and there is a need to address these.

For example, FedDF utilized average logits and FedET did weighted average.

thus further limiting the effectiveness of knowledge transfer and underscoring the need for a more adaptive and nuanced approach to knowledge distillation in federated learning settings.

- in reality devices vary in size and strength. prior works treat them equality important .. dilute the information that is beining transfered
furthermore, they use this same soft-target distillation to every student which is xyz -- using same target distillation may not be effective for training every student as each student has different learning capacity and ...
- therefore they lead to suboptimal knowledge transfer

 the primary focus in these works lies in

 To the best of our knowledge, this has not been previously explored.
 The success of KD, efficacy, suboptimal KD 
 
In these settings they face several challenges:
they lack support for knowledge transfer in diverse heterogeneous devices. do not fully address the challenges of knowledge transfer in settings with device heterogeneity. 


well-performing algorithms, it fails to take into account the intrinsic
diversity of the predictions of t

these methods cannot properly transfer knowledge in real-world settings.

% limiting the feasibility of training various model architectures.

Recently, task arithmetic technique has appeared as a promising technique in editing the knowledge of pre-trained models. 
\end{comment}

\begin{figure}
    \centering
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=0.75\linewidth]{nfigs/problem_a.png}
        \caption{Device Heterogeneous FL}
        \label{fig:sub1}
    \end{subfigure}
    \hspace{0.03\textwidth}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{nfigs/problem_b.png}
        \caption{AvgLogits}
        \label{fig:sub2}
    \end{subfigure}
    \hspace{0.008\textwidth}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{nfigs/problem_c.png}
        \caption{Our Approach}
        \label{fig:sub3}
    \end{subfigure}
    \caption{\textbf{Distinction of our approach.} (a) shows an overview of device heterogeneous FL where heterogeneous device prototypes with their unique configuration participate in FL. (b) prior works usually ignore that fact that heterogeneous  ensembles may vary in strength and helpfulness significantly and average all logits. (c) in our approach we consider each ensemble distillation as a task and edit the student model with task arithmetic.}
    \label{fig:main}
\end{figure}

\begin{comment}
Despite these advancements, current knowledge distillation (KD)-based methods in device heterogeneous FL are primarily designed for scenarios involving same-size device prototypes with similar capabilities and architectures. However, these methods fall short in establishing effective knowledge transfer when applied to real-world settings where device prototypes span a broad range of sizes and capabilities, from small IoT devices to large workstations. This shortfall arises primarily due three reasons: 
(1) Existing methods often disregard the individual strengths and information quality of each device prototype's ensembles and merge their logits into a single distillation target. This approach dilutes the richer, more informative logits from more capable devices with less informative outputs from less capable ones. Such integration fails to fully leverage the unique contributions of each device prototypes, particularly the more capable ones, and can potentially degrade the quality of the knowledge being transferred. 
(2) Additionally, these methods use this single integrated distillation target to guide knowledge transfer across all student models, regardless of their size. This one-size-fits-all approach does not account for the differences in architecture and learning capacities among the device prototypes' student models. Consequently, it fails to provide a customized distillation strategy tailored to each student model, based on their specific learning capacities and architectural differences.
(3) Furthermore, the ensemble distillation process can inadvertently lead student models into erroneous directions, causing them to forget their own knowledge acquired through locally updated parameters. This issue arises due to the inherent noise in the ensembles' logits, which are inferred on a public dataset unfamiliar to their original training data, compounded by the lack of supervision from the actual private datasets that are the primary learning objectives.
\end{comment}

\begin{comment}
In this paper, we propose a novel KD-based device heterogeneous federated learning framework, called FedHD to address the critical limitations of prior works and provide a more effective knowledge transfer for the more realistic scenarios where device prototypes varying capabilities. Inspired by the recent advancements in model editing via task arithmetic, we propose a novel knowledge transfer and integration framework which enables students to strategically customize the knowledge that is being transferred from each device to achieve more effective knowledge. To do so, we consider the knowledge transfer from each individual device prototype's ensembles as separate tasks. This way ensure that the unique knowledge of each device is being effectively distilled and is not being diluted or transformed by other devices. Furthermore, we introduce a self-regularization technique to this individual knowledge transfer process in order to protect the student from being drifted into erroneous directions and forget its own knowledge due to the noisy distillation as ensembles' logits are evaluated on an unfamiliar public dataset, distinct from their original training data and the distillation lacks supervision from the actual private datasets, which are the ultimate learning objectives. Subsequently, to merge the distilled knowledge from heterogeneous device prototype's ensembles we propose an adaptive task arithmetic operation, where the merging coefficient of each knowledge transfer task determine the amount of knowledge that is being integrated into student model. These merging coefficients allow the student to have selective knowledge transfer based on the helpfulness of each device and its own learning capacity and thus leading to more effective knowledge transfer and integration.



we extend the concept of task vectors to federate learning, by conceptualizing the averaged locally updated parameters as the pre-trained parameters in centralized learning, and the distilled parameters as the fine-tuned parameters.
Inspired by the recent advancements in model editing via task arithmetic in centralized learning, we construct task 

To achieve so, we extend the concept of task vectors to FL setting, by conceptualizing the averaged locally updated parameters as the pre-trained parameters in centralized learning, and the distilled parameters as the fine-tuned parameters.

have customize knowledge integration for each student model, we propose a novel knowledge integration technique inspired by the recent advancements in model editing via task arithmetic in centralized learning settings. Specifically, We extend the concept of task vectors to FL setting, by conceptualizing the averaged locally updated parameters as the pre-trained parameters in centralized learning, and the distilled parameters as the fine-tuned parameters. This allows us to form task vectors for each specific knowledge transfer tasks and merge them via task arithmetic operation. The merging coefficient of each task allows the student to have 


Drawing inspiration from recent advances in model editing through task arithmetic, we propose a unique knowledge transfer and integration framework. This framework empowers students to strategically customize transferred knowledge from each device, ensuring more effective knowledge acquisition. To achieve this, we treat knowledge transfer from each device's ensembles as separate tasks. This approach guarantees that the distinctive knowledge of each device is accurately distilled, without being diluted or altered by contributions from other devices.

%In particular, Instead of integrating the knowledge of all heterogeneous ensembles and distilling it into the students, we consider the knowledge transfer from each individual device prototype's ensembles as separate tasks. We further improve this individual knowledge transfer process by adding a self-regularization technique to protect the student from noisy we form a separate knowledge transfer process from each individual device prototype.  This way ensure that the unique knowledge of each device is being effectively distilled and is not being diluted or transformed by other devices. Furthermore, the ensemble distillation process may adversely impact the student due to two reasons: (1) ensembles' logits are inherently noisy since they are inferred on an unfamiliar public dataset, distinct from their original training data. The presence of data heterogeneity and insufficient training of some ensembles due to limited computational resources can further exacerbate this noise. (2) The distillation lacks supervision from the actual private datasets, which are the ultimate learning objectives. In order to protect the student from these issues and being drifted into erroneous directions and forget its own knowledge we introduce a self-regularization technique into this framework. Our self-regularization technique mitigate these issues by enforcing similarity between the logits of the student and its initial logits. We treat each knowledge transfer as a task. In order to integrate the knowledge from ensembles of heterogeneous device prototypes, we propose a novel task arithmetic approach. 

%take a substantial step forward by considering an important underexplored and more realist device heterogeneous FL where device capabilities vary span from small to large. We present a novel federated learning for heterogeneous device prototypes in FL, address these critical limitations of prior works. In this framework, 

%underexplored scenario where devices exhibit varying capabilities, ranging from small IoT devices to large workstations. 
\end{comment}

==> nsecs/introduction.tex <==
\section{Introduction}

% Therefore, it is essential to consider cross-device \textbf{device heterogeneity} settings in FL, where each device has different architecture, computation resource and memory size

%the performance improvement of federated learning by either excluding lower-end or higher-end devices or reducing the 


% In reality there exists a diverse spectrum of device types, from small ones such as IoT devices and smartphones to large ones like desktop computers, and supercomputers with different computing power and memory size. 

%Fedavg has become the de-facto federated learning algorithm and has been used in many applications. However, 

%setting significantly limits the performance improvement of federated learning models by excluding lower or higher-devices who would make noticebale contribution to the model training from their local data.

The proliferation of edge devices, such as IoT devices and smartphones, has propelled them into becoming primary platforms for computing and machine learning tasks. These devices host vast and diverse datasets, which are invaluable for enhancing machine learning models. Yet, the sharing of such data with third-party users raises significant privacy concerns among users. To address these privacy concerns, federated learning (FL) has emerged as a promising distributed machine learning paradigm. FL enables the collaborative training of a shared global model across multiple clients while preserving the privacy of each client's local data. 
The majority of existing works in FL predominantly focus on cross-device \emph{device-homogeneous} settings where all clients are assumed to have the same computation power and can train an identical global architecture. However, this assumption limits the potential of collaboration among heterogeneous devices with different computing power and memory size which can significantly contribute to model performance improvement with their unique local data. Therefore, to fully harness the diverse capabilities of edge devices and leverage their unique data contributions to improve model performance it is essential to consider cross-device \textbf{device heterogeneity} settings in FL.

The primary challenge in device heterogeneous FL is how to aggregate heterogeneous client models? To address this, prior research has explored two different settings and proposed methods for their device heterogeneous FL settings. Some studies have aimed device heterogeneous setting where a single global model is being trained and heterogeneous sub-models of this single global model is deployed across clients depending on their system resources. These studies proposed sub-model extraction techniques to address this device heterogeneous FL setting. However, this setting is not practical since clients often possess unique model architectures optimized for their specific hardware, software and dataset. Alternatively, other works have considered device heterogeneous settings where some fixed architecture prototypes are evenly assigned to the clients at random and adopted knowledge distillation with a public dataset methods to improve each model prototype.

In this work, we present a more general device heterogeneous setting in FL inspired by the real-world scenarios. In reality there exists a diverse spectrum of device types, from small ones such as IoT devices and smartphones to large ones like desktop computers, and supercomputers with different architectures, computing power and memory size. Naturally, these devices can be grouped into clusters based on their types, with each cluster exhibiting differences in architecture, number of clients, and dataset size. For instance, smartphones typically feature numerous clients, smaller architectures, and datasets compared to desktop computers. It's noteworthy that the device heterogeneous setting considered in prior works, as discussed earlier, is a specialized case of our new setting. In our setting, the number of clients and dataset sizes may vary across clusters.

We empirically analyze the prior KD-based methods in this generalized device heterogeneous setting. Our empirical analysis reveals that the existing methods including FedDF and Fed-ET face significant challenges. Specifically, we make several observations: (1) The performance of KD-based methods declines when dataset sizes per clusters are uneven. (2) Similarly, uneven numbers of ensembles per cluster negatively affect KD-based methods' performance. (3) Heterogeneity in architecture families across clusters also leads to reduced performance. (4) Increasing domain differences between public and private datasets adversely affect KD-based methods' performance, as the ensemble distillation process may direct models inaccurately. Furthermore, challenges 1-3 stem from improper ensemble weighting in the knowledge distillation process. While FedDF employs uniform ensemble weighting, some ensembles provide more assistance. Conversely, Fed-ET's ensemble weighting based on logit confidence can result in biased distillation and reduced model generalization as shown in xxx. Challenge 4 comes from the fact that as the domain difference increases, the logits become more erroneous and thereby, the ensemble distillation process may direct the models into inaccurate directions.

Motivated by these insights, we propose \textbf{FedHD} (\textbf{Fed}erated Learning for \textbf{H}eterogeneous \textbf{D}evices), a novel KD-based framework that accommodates clusters of heterogeneous devices in FL. In FedHD, heterogeneous ensembles (client models) act as teachers, transferring knowledge to cluster-specific global models (students) using a public unlabeled dataset at the server. For each cluster's global model training, FedHD combines heterogeneous ensemble distillation objectives using an adaptive weighting scheme based on ensembles' model and dataset sizes. This scheme capitalizes on the intuition that smaller models benefit more from larger ones, while the reverse is less true.
Additionally, challenge 4 stems from the fact that domain differences between public and private datasets introduce noise and unreliability in ensemble logits. To mitigate this, we introduce a self-guarded regularization term to preserve each cluster's global model's initial logits on the public dataset during ensemble distillation. We empirically evaluate FedHD on two architecture settings: "homo-family," where cluster models share the same architecture family, and "hetero-family," where they may not. Our experiments on CIFAR-10 and CIFAR-100 datasets demonstrate FedHD's state-of-the-art performance in both settings, showcasing its effectiveness in addressing the introduced problem.


% In the past, there have been some works attempt to devise \emph{model-heterogeneous} FL algorithms, inwhich the focus is mainly on allowing clients to train heterogeneous models based on their computation power. Some works propose knowledge distillation (KD) techniques~\cite{hinton2015distilling}, where they distill different size ensemble's logits on a public dataset into a larger~\cite{cho2022heterogeneous} or multiple models~\cite{lin2020ensemble, sattler2021fedaux} at the server. Some other works propose partial model training (PT) techniques, where clients are tasked with training sub-models extracted from the global model based on their computational capabilities~\cite{diao2020heterofl, alam2022fedrolex, horvath2021fjord}. 


In summary, our paper make the following key contributions:


%To support device heterogeneity in FL, prior works have explored mainly two settings. Some works considered training a single global model is being trained and propsed partial model training techniqeus where clients are tasked with training sub-models extracted from the global model based on their computational capabilities. However, in practice clients may have their own unique model architecture optimized according to their specific hardware and software and tuned to give best performance on their specific task and dataset. Other works, consider clients to have their own model architecture and proposed transferring knowledge between clients model architecture using ensemble distillation with a public dataset at the server.

%To address limitations of device-homogeneous settings in FL, several works have extended the setting to include clients with heterogeneous architectures. The prior works mainly considered two settings: (1) 

%The main challenge in device heterogeneous FL is To address device heterogeneity

%Inspired by the practical realworld case where there are different device types, we consider a new device-heterogeneity setting by considering federated learning between different device types. 


% Recently, it is has been shown that large models have huge capabilities, however they cannot be deployed in FL by small devices. Therefore, it is also needed to have advanced FL algorithms which large models accomodated at large devices can be benefitted by small models in FL. 

%the sizes of the ensembles
%Unlike FedDF, which treats every ensemble equally and simply averages all the logits to form a single ensemble distillation loss, we adopt a different approach.

%However, this concentration limits the potential of collaboration among a diverse range of devices, each possessing its unique, unhashable model, memory capacity, and computational power, all of which can significantly contribute to model performance. In this study, we take a a substantial step forward by defining a new problem wherein various classes of devices, each possessing distinctive models, memory capacities, and computational resources, collaborate to enhance each other's global model within the federated learning paradigm

%Such unrealistic settings can only include a specific class of devices such as smartphones with the same  The main challenge in model-heterogeneous FL is inability to aggregate the parameters of clients. 
%In the past, there are some prior works attempting to design model-heterogeneous FL algorithms where clients are allowed to train heterogeneous models according to their resource constraints. These works fall into two categories: (1) Knowledge Distillation (KD) and (2) Partial Model Training (PT). Works in the first (KD-based) approach propose ensemble distillation using a public dataset to train single or multiple global model at the server. For example, FedDF~\cite{lin2020ensemble} introduced ensemble distillation by using Kullback-Leibler (KL) divergence loss between the averaged logits of ensembles and the global model's logits which works well on data heterogeneity settings. However, this does not work well when there are different size models since all ensembles from small to large are being weighted equally. The works in the second approach (PT-based), clients train an extracted sub-model of the global model according their computation power. For example, HeteroFL and FjORD uses a static sub-model extraction while FedRolex relaxes this condition and proposes a rolling sub-model extraction. However, in reality different class of devices have their own designed model architecture tailored to their specific hardware and software system and may not be able to train different model architectures. Also, these approaches suffer from sub-models interference and not being balanced which makes aggregating them and putting them back into the global model difficult.

%A noteworthy distinction that sets FL apart from centralized training is its ability to encompass a diverse spectrum of devices, ranging from smartphones, IoT devices, computers, to data centers, within the learning process. However, the strength of this diversity also presents a challenge due to the highly heterogeneous nature of these devices. They significantly vary in computation power, memory capacity, communication bandwidth, size of their local dataset, and  availability to actively participate in the FL procedure.
%\textbf{device-heterogeneity} 


==> nsecs/limitations.tex <==
\subsection{Limitations}
In this work, we introduced TAKFL, a novel federated learning framework designed to facilitate effective knowledge transfer across a spectrum of heterogeneous device prototypes. While our experiments simulate a real-world environment by considering a range of device sizes, the actual deployment on physical devices remains untested. Experiencing TAKFL in real-world settings could provide additional insights and possibly highlight unforeseen challenges or limitations.

Moreover, our current study is confined to image classification and text classification tasks. The effectiveness of TAKFL in handling more complex tasks such as image segmentation, text summarization, or question answering remains unexplored. Extending our framework to these areas could reveal task-specific challenges and may necessitate modifications to the distillation and integration strategies used in TAKFL.

Additionally, while TAKFL shows promise in scenarios involving a limited number of device sizes, its scalability and efficiency in environments with an extremely large and varied number of devices have not been thoroughly evaluated. This scalability is crucial for broader applicability in real-world federated learning scenarios where device characteristics can vary widely.

These limitations underscore the need for further research to fully realize the potential of TAKFL and to ensure its adaptability and robustness across different domains and in actual deployment scenarios.

==> nsecs/oldnotes.tex <==
\paragraph{Older Notes, move later}

Consider now two models, with $\btheta_{avg}^{1}\in\Theta^1:=\argmin{\btheta} \sum\limits_{k\in \C^1} 
\mathbb{E}_{(\bx,y)\sim \D^1_k}\left[ \ell (f^1(\bx;\btheta),y) \right]$ and likewise for $\btheta_{avg}^2$. Furthermore, in the notation of Assumption~\ref{as:zerolossas1}, assume that $D_1$, $D_2$ and $M_1=M_2$ for prototype $1$ and prototype $2$, respectively. We denote their tangent projectors as by, e.g. $\Sigma^1_{\parallel}$. Finally, assume that the server has access to the distribution $\mathcal{D}' = \omega_1\mathcal{D}^1_{\epsilon}+\omega_2\mathcal{D}^2_{\epsilon}$ with $KL(\mathcal{D}^1,\mathcal{D}^1_{\epsilon})\le \epsilon$ and $KL(\mathcal{D}^2,\mathcal{D}^2_{\epsilon})\le \epsilon$. 


Now, the server would like to, ideally, train, to develop a model for device prototype 1 that fits both its and prototype 2's data,
\[
\argmin{\btheta} \sum\limits_{k\in \mathcal{C}^1_{\epsilon}\cup\mathcal{C}^2_{\epsilon}} 
\mathbb{E}_{(\bx,y)\sim \D^1_k}\left[ \ell (f^1(\bx;\btheta),y) \right]
\]
Of course, this is not possible, but we can consider the federated learning procedure as an attempt to achieve some approximation of this. 

%To perform the connection more explicitly, we define the original training objective function of interest
%to involve four clients, without considering multiple private local datasets. That is:
%\[
%\min_{\theta^1,\theta^2,\theta^3,\theta^4}\, \sum\limits_{j=1,..,4} \mathbb{E}_{(x,y)\sim \mathbb{D}^j}\left[l(f^j(x;\theta^j),y)\right]
%\]
%Let us consider that $\theta^1,\theta^2\in\mathbb{R}^{D_1}$ and $\theta^3,\theta^4\in\mathbb{R}^{D_2}$ are smaller and larger models, respectively. 
%Let us write $Y^1,Y^2,Y^3,Y^4$ to be the stochastic processes defining the gradient flow that we consider as reaching the corresponding
%minimizer manifold $\Gamma^j$. 

We can formulate the Vanilla Distillation procedure as:
\[
\hat{\btheta}^1_{VD} \in \min KL\left(f^2(\bx;\hat{\btheta}^2_k)\vert\vert f^1(\bx,\btheta^1)\right)
\]
which can be written as:
\[
\hat{Y}^1_{VD}\in \min KL(Y^1 \vert\vert Y^2)
\]
which will have a solution unrelated to the subspace decomposition of $Y^1$ and $Y^2$. 

Now consider the circumstance wherein, theoretically the two devices cooperate to solve, together,
\begin{equation}\label{eq:coop}
\hat{Y}^1,\hat{Y}^2 \in KL(Y_1 \parallel Y_2)+KL(Y_2\parallel Y_1)
\end{equation}
which would clearly yield a better solution. Of course, this cannot be done in practice, but we will now demonstrate that the properties of task arithmetic are aligned with solving this cooperative problem. 

Consider a candidate solution $\hat{Y}$ for which $\hat{Y}$ satisfies~\eqref{eq:sdesoln}, with $\Sigma_{\hat{\parallel}}$ given by 
\[
\Sigma_{\hat{\parallel}} = \Sigma^1_{\hat{\parallel}}\cap \Sigma^2_{\hat{\parallel}} 
\]
This would minimize the divergence in the tangent direction, and would a reasonable low objective solution for~\eqref{eq:coop}. 

Now, let us consider the impact of the prototype device capacity. In particular, we compare the circumstance wherein $\dim\left(\Sigma^1_{\hat{\parallel}}\right)=\dim\left(\Sigma^2_{\hat{\parallel}}\right)$, corresponding to $D_1=D_2$, and $\dim\left(\Sigma^1_{\hat{\parallel}}\right)<\dim\left(\Sigma^1_{\hat{\parallel}}\right)$, corresponding to $D_1>D_2$. 

\textbf{Case 1:} Consider an eigenbasis for $\Sigma^1_{\hat{\parallel}}$ and then expand it to $Y^1$ as $\{e^1_l\}_{l=1,...,M_1}$. Consider the procedure of picking an eigenvector of the basis of $Y^1$ uniformly at random without replacement and note that there is a $(D_{1+s}-M_{1-t})/M_{1-t}$ chance any particular eigenvector belongs to $\Sigma^1_{\hat{\parallel}}$, where $t$ is the number of trials in the sampling and $s$ is the number of ``hits'' so far. Let us compute the expected number of subspaces in common. This would correspond to the relative computational ease (that is, with an increasing dimension) of KD. We have that the expectation can be defined through the combinatorial operator $\mathop{Ch}(n,p)=\frac{p!(n-p)!}{n!}$
\[
\sum\limits_{i=0}^{D-M)} i \frac{\mathop{Ch}(M,i)}{2\mathop{Ch}(M,D-M)}
\]
For, e.g., $D=3$ and $M=1$ this is $\frac{1}{2}$.

\textbf{Case 2:} In this case, we can compute the expectation to be:
\[
\sum\limits_{i=0}^{D_1-M)} i \frac{\mathop{Ch}(M,i)}{\mathop{Ch}(M,D_1-M)+\mathop{Ch}(M,D_2-M)}
\]
For, e.g., $D_1=3$ and $M=2$ this is $\frac{1}{2}$.

From what we can see, there is a more than linear drop in the total dimension available for a KD optimization problem to approximate, thus providing a model for the phenomenon that learning from models with larger device prototype with task vector KD should be prioritized for federated learning. 

%Note that since $dim\left(\Sigma^1_{\parallel}\right)<dim\left(\Sigma^2_{\parallel}\right)$ it may be preferable still to make $\Sigma_{\hat{\parallel}} = (\Sigma^1_{\hat{\parallel}}\cup v)\cap \Sigma^2_{\hat{\parallel}} $ for some vector $v$ not in the span of $\Sigma^1_{\hat{\parallel}}$ but in the span of $\Sigma^2_{\hat{\parallel}}$, in order to expand the dimensionality of the model.






==> nsecs/revisit.tex <==
\section{Background: Federated Ensemble Distillation}
\textcolor{red}{In this part, we revisit the prior federated ensemble distillation as a necessary background and preliminary.}

\subsection{Knowledge Distillation}
Consider a $K$-way classification problem on a dataset $D = \{(\bx, \by) \vert \, \bx \in \cX, \, \by \in \cY \}$, where $\cX \subseteq \reals^D$ is the feature space and $\cY \subseteq \{0, 1, \cdots, K\}$ is the set of labels. Furthermore, Let $\cT$ be a pre-trained teacher model and $\cS_{\btheta}$ a student model. Knowledge distillation (KD)~\cite{hinton2015distilling}, distills the teacher's knowledge into the student model by encouraging the student to mimic the behavior of the teacher. This is achieved by minimizing the Kullback-Leibler divergence between the student's softened logits and those of the teacher on a input data $\bx$, as following:
\begin{align*}
\mathcal{L}_{KL} = KL\left[\sigma\left(\cT(\bx)\right) \, \Vert \, \sigma\left(\cS_{\btheta}(\bx)\right)\right].
\end{align*}
In the above equation, $\sigma$ represents sotfmax function with temperature $T$ defined as $\sigma(\bz)_i = \frac{\exp(z_i / T)}{\sum_j \exp(z_j / T)}$, and $KL$ represents the Kullback-Leibler divergence loss.

\subsection{Task Arithmetic.}
A task $t$ is defined as a specific instance of a dataset paired with a corresponding loss function. For any given task $t$, a task vector is derived by subtracting the model's pre-trained weights $\btheta_{pre}$ from its fine-tuned weights $\btheta_{ft}^t$ on task $t$ , i.e. $\tau_t = \btheta_{ft} - \btheta_{pre}$. To construct a model that performs adeptly across multiple tasks $\{\tau_t\}_{t=1}^{T}$, the task vectors are aggregated and then applied to the pre-trained model weights, resulting in $\btheta = \btheta_{pre} + \lambda \sum_{t=1}^T \tau_t$. Here, $\lambda \in [0,1]$ serves as a hyperparameter that controls the extent of model adaptation. Task arithmetic offers a straightforward, cost-efficient, and scalable method for model editing, demonstrating superior performance compared to methods such as weight averaging.

\subsection{Federated Ensemble Distillation}
Standard FL methods, like FedAvg~\cite{mcmahan2017communication}, face a significant limitation in solving eq~\ref{eq:problem}. Specifically, they are designed to operate independently for each device prototype and lack the capability to accommodate heterogeneous devices with varying neural network architectures and thereby unable to harness the potential data value of heterogeneous devices which is essential for performance improvement. To address this limitation, \citet{lin2020ensemble} proposed ensemble knowledge distillation to transfer knowledge between heterogeneous devices in FL.

%ensemble knowledge distillation has appeared as a promising approach to transfer knowledge between heterogeneous devices in FL~\cite{lin2020ensemble, mora2022knowledge, li2024federated}.

%\citet{lin2020ensemble} proposed a knowledge distillation framework in order to resolve this limitation which transfers the knowledge across heterogeneous devices using ensemble knowledge distillation.

In this context, at each round $r$ a subset of clients $\C^{j}_r$ from each device prototype $j \in \M$ is randomly selected by the server and download their corresponding model initialization $\btheta_r^{j}$. Each client $c_k^{j} \in \C^{j}_r$, starting from this model initialization, locally train the model $f^j$ on its local private data $\D^j_k$ by taking multiple steps of stochastic gradient descent. Then, they send back their updated parameters $\{{\widehat \btheta^j_k}\}_{k \in \C^j_r}$ to the server. The server aggregates the received clients parameters, computing $\btheta_{avg}^j = \sum_{k \in \C^j_r} \frac{\l \D_k \l}{\sum_{k \in \C^j_r} \l \D_k \l} {\widehat \btheta^j_k}$ to initialize each server model $f^j$. Subsequently, each each server model $f^j$ starting from this initialization, undergoes updates using ensemble knowledge distillation. 
Here, heterogeneous client models from heterogeneous devices, collectively termed as ensembles, i.e., $\btheta_{ens} = \{\widehat \btheta^{i}_{k} \vert \, i \in \M, \, k \in \C^i_r\}$, serve as teachers, transferring their knowledge to each server student models $f^i(\cdot, \btheta^i)$.

Specifically, let $\bx \in \D^{public}$ be a mini-batch of data from an unlabeled public dataset, and $\bz^i_k = f^i(\bx;\btheta^i_k)$ denote the logits of ensemble $\widehat \btheta^i_k$, while $\bq^i = f^i(\bx;\btheta^i)$ denote the logits of device prototype $m_i$ server student model. For simplicity, we drop the index for each server student model, denoting it as $\bq = f(\bx;\btheta)$. Consequently, the softened averaged logits of the entire ensemble are considered as the soft target for distillation, aiming to teach each server student model. This objective is captured by the following equation:
\begin{align} \label{eq:ed}
\small
\hspace{-1.7mm}\mathcal{L}_{\text{ED}} = \text{KL}\bigg[\sigma\bigg(\frac{1}{\sum_{j \in \M}\vert\C^j_r\vert} \sum_{j\in \M}\sum_{k \in \C^j_r} \bz^i_k \bigg) \, , \, \sigma\left(\bq\right)\bigg]. \quad \text{(AvgLogits)}
\end{align}

FedDF~\cite{lin2020ensemble} uses the AvgLogit objective defined in equation~\ref{eq:ed} to update every heterogeneous server student models. However, this approach has two significant limitations: \textcircled{\small 1} in practice, there exist different size device prototypes from small ones with small data and small model to large ones with large data and large models where they vary in strength significantly. Therefore, the teacher ensembles coming from different size device prototypes vary in strength and helpfulness significantly. AvgLogits neglects this fact and equally regard the importance of all teacher ensembles in the knowledge distillation which may be suboptimal. For instance, consider a federation involving a smartwatch and a desktop computer. The ensembles from the smartwatch, due to its small dataset and model size, are inherently weaker compared to those from the desktop computer. Nevertheless, AvgLogits disregards this distinction and combines the logits of both weak and strong ensembles without consideration of their relative strengths. \textcircled{\small 2} FedDF employs the same soft distillation target for knowledge transfer across different server student models, utilizing the AvgLogits objective in equation~\ref{eq:ed} for all. However, student models vary in size, learning capacities, and architecture significantly. Consequently, using the same soft target distillation may not facilitate an optimal knowledge transfer. Each server student model may require a tailored distillation target to effectively leverage the knowledge embedded in the teacher ensembles.
To clarify, let's consider our previous example involving a smartwatch and a desktop computer. The smaller smartwatch student model may derive greater benefit from distilling knowledge from the larger ensembles of desktop computers. Conversely, the larger desktop computer student model may struggle to effectively learn from smaller teacher ensembles due to their limited knowledge and capacity. 

% Consequently, using a uniform soft target for distillation may not facilitate optimal knowledge transfer. Each server model may require a tailored distillation target to effectively leverage the knowledge embedded in the teacher ensembles.

% These issues are well-studied in knowledge disillation literature as transfer gaps~\cite{zhu2021student, cho2019efficacy, niu2022respecting}.

% Prior works have used the same soft distillation targets (
% - we may have more number of weak ensembles than strong ones.
% - fedet uses uncertainty-weighted distillation. issues with fedet?
% - over-confidence of weak ensembles. fedet may not address this.

% \begin{proposition}\label{prop1}
% In ensemble knowledge distillation, the KL divergence between averaged softened logits of ensembles and the softened logits of the teacher is equivalent to the averaged KL divergencen between each ensemble's logits and the teacher's logits.
% \end{proposition}

% \begin{proof}
% To prove it .
% \end{proof}

%  the knowledge as model initialization to update the server-size model through the ensemble distillation. 

% Suppose there is a set of clients $S$, where each client $k$ has local dataset $D_k$. The entire clients participate in federating learning process to train a machine learning model $f(\cdot; \btheta)$ over the whole dataset $\cD = \bigcup_{k=1}^{\l S\l} \cD_k$ under orchestration of a central server while preserving the privacy of local datasets. At each round $r$, $C \in (0, 1]$ fraction of clients are being randomly selected denoted as $S_r$. The $S_r$ selected clients receive the current parameters of global model $\btheta_r^g$ and locally train it. Then, they send back their updated parameters $\{{\widehat \btheta_k}\}_{k \in S_r}$. Consequently, the server updates the global model by aggregating the locally updated parameters $\btheta_{r+1}^g = \sum_{k \in \l S_r\l} \frac{\l \cD_k \l}{\sum_{k \in \l S_r\l} \l \cD_k \l} {\widehat \btheta_k}$. This process continues for $R$ communication rounds.

% One round of federated training is then performed as follows: A subset St of the client population is selected by the server and downloads a model initialization. Starting from this model initialization, each client then proceeds to train a model fi on it’s local private data Di by taking multiple steps of stochastic gradient descent. We assume that these local models can be decomposed into a feature extractor hi and a classification head gi according to fi = gi ◦ hi. Finally, the updated models fi, i ∈ St are sent back to the server, where they are aggregated to form a new server model f , which is used as the initialization point for the next round of FL. The goal of FL is to obtain a server mode
